MRI Reconstruction with Regularized 3D Diffusion Model (R3DM)

Magnetic Resonance Imaging (MRI) is a powerful imaging technique widely used for visualizing structures within the human body and in other fields such as plant sciences. However, there is a demand to develop fast 3D-MRI reconstruction algorithms to show the fine structure of objects from under-sampled acquisition data, i.e., k-space data. This emphasizes the need for efficient solutions that can handle limited input while maintaining high-quality imaging. In contrast to previous methods only using 2D, we propose a 3D MRI reconstruction method that leverages a regularized 3D diffusion model combined with optimization method. By incorporating diffusion based priors, our method improves image quality, reduces noise, and enhances the overall fidelity of 3D MRI reconstructions. We conduct comprehensive experiments analysis on clinical and plant science MRI datasets. To evaluate the algorithm effectiveness for under-sampled k-space data, we also demonstrate its reconstruction performance with several undersampling patterns, as well as with in- and out-of-distribution pre-trained data. In experiments, we show that our method improves upon tested competitors.

==> Section/discussion.tex <==
\section{Discussion}\label{sec:discussion}

==> Section/introduction_old.tex <==
\section{Introduction} \label{sec:intro}
% Importance of MRI imaging; inefficiency; solution

% the need for 3D reconstruction
% CZ: here we need to list, for example, GRAPPA, UNet
% Given that the 3D model is data-hungary, we observe that out-of-distribution performs good.
In order to speed up the acquisition time, MRI measurements use sub-sampled k-space. Several attempts have been made to develop methods for sub-sampled k-space, as discussed in \cite{zbontar2018fastmri,muckley2021results, dwork2021fast, chung2022score}, where the proposed algorithms are shown to have the capability to reconstruct the image from various types of under-sampled k-space data. %acquisition 
Given that the MR images are acquired slice by slice, most works focus on reconstructing the two-dimensional (2D) slices and then stacking these slices to form a three-dimensional (3D) volumetric image. This method doesn't consider the inter-dependency between the slices, it can lead to inconsistencies and artifacts, as discussed in \cite{chung2023solving, banerjee2021completely, wu20203d}. 
Many datasets have particularly noticeable artifacts due to the equally distributed information and structures with high continuity on all dimensions, such as roots and vessels\cite{schulz2013plant, wu20203d, banerjee2021completely}.
% Although some MR measurements are designed only to have rich information on slices (\eg the fastMRI knee data \cite{zbontar2018fastmri}), 

The extension by stacking 2D diffusion model-based reconstruction to get a 3D image has been investigated, for instance in \cite{chung2023solving}. The method can be seen as a two-stage process by generating 2D images from pre-trained networks as in \cite{chung2022score} and using an optimization method and regularization techniques to help produce consistency in the sequence of 3D images. 
However, extending the 2D model into 3D also improves the representation by capturing volumetric information with higher precision to describe the details of the object under observation, as discussed in \cite{wu2021denoising}.
This enhancement contributes to a more comprehensive understanding of the underlying data, making the model perform much better than its 2D counterpart. 
% In such cases, a 3D model is needed to capture volumetric information with higher precision to describe the details of the object under observation. 

Training and sampling a 3D Diffusion Model is computationally expensive. As highlighted in \cite{voleti2022mcvd}, the 2D U-Net with cross-attention on the 3rd dimension (the 2D+T architecture hereafter) is more efficient than the 3D U-Net version for video data generation. Aligning with the fact that MR images are taken sequentially, the 3rd dimension of MR images can be regarded as the temporal dimension. 
% To avoid performance drop introduced by the limitation of the architecture, we further propose to use axis projection acquired by the Fourier slice theorem (FST) \cite{bracewell1990numerical}, which gives the relation between the axis projection of 3D volume images in MRI and zero-frequency in the under-sampled k-space.

% Contribution (what we propose)
To summarize, we propose a new method to address the inconsistency problem of 3D MRI reconstruction with sub-sampled k-space measurements. The method considers the 3D representation of MR images without using expensive 3D models. The workflow is summarized in \Cref{Fig:workflow}  and our contributions are summarized below:
\begin{itemize}

% \item We propose an optimization algorithm based on the Fourier slice theorem (FST) \cite{bracewell1990numerical}. Instead of reconstructing the image slice by slice, the algorithm allows us to perform direct reconstruction on volume images using a diffusion model that captures 3D representation.
\item We propose an optimization algorithm to improve the MRI reconstruction quality of video diffusion models used for 3D MRI reconstruction.
\item We demonstrate that the 3D representation is important for 3D MR reconstruction by performing numerical experiments to compare the performance of the proposed algorithm against state-of-the-art algorithms. We measure the quality of image reconstruction based on several well-known metric evaluations, such as \ac{SSIM} and \ac{PSNR} for both in- and out-of-distribution data. Additionally, the ablation studies to measure the effect of all parameters are also observed. All code used in this paper will be available.
%\textcolor{blue}{the link here}
\end{itemize}

% , such as the BRATS \cite{menze2014multimodal}  and Plant Root data. 


% Advancements in 3D MR imaging methods can address the challenges posed by complex anatomical structures of human organs and plant growths. Consequently, the demand for developing 3D MR image reconstruction methods has intensified. 

 
% This approach is feasible because each slice has a unique k-space measurement that can be used to construct the 3D image. 

%   The problem becomes more pronounced if one considers sub-sampled k-space to construct 3D volume images in MRI, due to the lost information during measurement processes. 

%information into the 3D Diffusion Denoising Probabilistic Method (DDPM) \cite{ho2022video} with the proximal projection method. We train a 3D diffusion model and propose an optimization method that uses under-sampled k-space measurement as a constraint to reconstruct 3D MR images with high fidelity.
% The Diffusion Model learns the prior knowledge of MR images to address the incomplete information due to under-sampled k-space.
% \item To address the incomplete information due to under-sampled k-space, we incorporate a diffusion model that learns the prior knowledge of MR images.
% that helps to generate initialization on the 3D image space. 
% As highlighted in \cite{voleti2022mcvd}, the 2D U-Net with cross-attention on the 3rd dimension (the 2D+T architecture hereafter) is more memory-efficient than the 3D U-Net version. This work shows that the 2D+T architecture also delivers strong performance for 3D MRI reconstruction.
% Here we perform training on the 2D + t U-Net architecture, for instance in \cite{ho2022video}, than 3D U-Net and 3D attention, as has been discussed in \cite{voleti2022mcvd} the latter requires excessively large amount of memory. 
% As highlighted in \cite{voleti2022mcvd}, the 2D+T U-Net architecture is significantly more memory-efficient than the 3D U-Net version. In this work, we show that the 2D+T architecture also delivers strong performance.
%\item We provide a trained 3D diffusion model implemented for MR reconstruction using our proposed method. We adopt and train the model implemented by on fastMRI knee data \cite{zbontar2018fastmri}.
% \section{Introduction}\label{sec:intro}
% % Importance of MRI imaging; inefficiency; solution
% Magnetic Resonance (MR) imaging is an imaging modality routinely used in clinical medicine, for instance, oncology, neurology, etc, due to the fact that it provides detailed anatomic imaging and can be used to help clinicians for diagnostic, monitoring, and treatment planning of the patients. However, the acquisition of a high-quality MR image is time-consuming, inconvenient for the patients, produces motion artifacts, and comes with high costs for the health system. In order to reduce scan time, the k-space domain in which MR images are acquired can be sub-sampled (e.g. the number of scan lines in the k-space domain can be reduced). While this procedure leads to shorter scan times, these sub-sampled data yield incomplete information and lead to noisy and disturbed images. Therefore, it is of high interest to develop algorithms that can generate high-quality images from under-sampled k-space data. Apart from the application in the clinical domain, MR imaging is also essential for plant phenotyping, i.e., investigation of plant roots, where it helps to disclose the structure of plants as well as to identify the characteristics of plants that can grow well under extreme climate conditions. This stems from the fact that MR imaging is a non-invasive imaging modality employed to observe the intricate structure of plant roots \cite{pflugfelder2017non, muhlich2008measuring, van2016quantitative}. Similar to the medical domain, a challenge arises in utilizing MR imaging techniques to capture the fine structures of roots from far less measurement data, due to their thin structure and low signal-to-noise ratio during acquisition of data.  
% \newline
% Conventional methods implemented in current MR scanners for accelerating data acquisition are e.g. parallel imaging and compressed sensing \cite{larkman2007parallel, pruessmann2006encoding, lustig2008compressed}. In parallel imaging, multiple receiver coils are used in the acquisition proces, where each coil receives an under-sampled amount of k-space data. The information of these coils and by incorporating estimated sensitivity maps for each coil, the information of these coils can then be merged to reconstruct one final image. For this purpose, algorithms such as SENSE and  GRAPPA are used \cite{pruessmann1999sense, griswold2002generalized}, where the process to fill the missing information either in image space or k-space are performed. While parallel imaging can accelerate the acquisition time by a factor of 2 or 3, the use of compressed sensing can accelerate the acquisition time by an even higher factor of about 4-8. Compressed sensing is using prior knowledge about the MR signal to iteratively minimize a data fidelity and a regularization term and reconstruct the undersampled k-space data to a high quality image.   \newline
% As the aforementioned methods have the limitations of e.g. defining the most suitable prior, the use of Deep Learning methods for MR image reconstruction becomes more and more popular \cite{terpstra2020deep, dar2020transfer,aggarwal2018modl,zhu2018image}. Hereby, traditional Convolutional Neural Networks (CNNs) with different architectures have demonstrated promising results such as e.g. the Automap framework \cite{zhu2018image} or other deep networks especially designed for MR image reconstruction \cite{eo2018kiki}. The development of deep learning-based MR image reconstruction is becoming prevalent due to the development of generative model, such as Generative Adversarial Networks (GAN), Normalizing Flows, Denoising Score Matching, and Diffusion Models \cite{mardani2018deep, yang2020pocs,zhang2018multi, song2021solving, chung2022score, wen2023conditional}, where it is demonstrated that those approaches can generate high-quality images from under-sampled k-space data. In this article, we will focus on the development of the diffusion model for image reconstruction. In general, both denoising score matching and the diffusion model \cite{hyvarinen2005estimation, ho2020denoising, song2020score} can be seen as a discretized version of continuous \ac{SDE} processes \cite{song2020score}, which depend on the growth of the noise variance over time. %Therefore, both cases are also called Variance Exploding (VE) and Variance Preserving (VP) \ac{SDE} \cite{song2020score}
% %GANs consist of a generator network generating the reconstructed images and a discriminator network that identifies 'fake' images, i.e. images that were generated from the generator network. In several papers, different GAN variants such as a least-squares GAN \cite{mardani2018deep}, cycle GAN \cite{yang2020pocs}, a multi-channel GAN \cite{zhang2018multi} generating high-quality images from under-sampled k-space data. \newline
% % \subsection{Related Works} 
% % While many proposed algorithms work on 2D MR image reconstruction, the demand for developing 3D MR image reconstruction methods has intensified. This arises from the need to capture volumetric information with higher precision to describe full information of the object under observation. For clinical as well as plant phenotyping, advancements in this area aim to address the challenges posed by complex anatomical structures of human organs and plant growths. Diffusion models have been applied for 3D MR image reconstruction in various works, for instance in  \cite{khader2023denoising, zhu2023make, chung2023solving}. 
% % In \cite{khader2023denoising}, the latent diffusion model-based 3D MR image reconstruction has been proposed, where instead of processing and training directly on the images, a mapping technique from Vector Quantized Generative Adversarial Network (VQ-GAN) \cite{esser2021taming} has been appended to Diffusion Denoising Probabilistic Method (DDPM) \cite{ho2020denoising}. 
% % Similarly, in \cite{zhu2023make}, the latent diffusion method \cite{rombach2022high} is used to map from the image space to the latent space. In general, the algorithm consists of two components: a latent diffusion model and volumetric layers. These components work together to reverse the process from latent space and generate volumetric data. 
% % The key idea in these studies closely resembles the generation of images without incorporating under-sampled k-space. Consequently, the images produced by such models can exhibit very high resolution, resembling MR images, but are independent of the specific data related to the acquisition process. 

% % K-space data plays a crucial role in reconstructing MR images, aligning with the unique aspects of the acquisition process. Incorporating under-sampled k-space data, the development of denoising score matching for 3D MR image reconstruction has been proposed previously, for example in \cite{chung2023solving}, where the reconstruction process has been combined with an optimization method. In general, the method can be seen as a two-stage process by generating 3D images from pre-trained networks as in \cite{chung2022score} and using an optimization method with additional information from under-sampled k-space. The k-space information is used as the data fidelity term to reconstruct consistent 3D images. Although the original work is trained for slice MR images, the optimization method and regularization techniques help to produce consistency in the sequence of 3D images. 

% % In this article, we propose 3D MR image reconstruction by using the Video Diffusion Denoising Probabilistic Method (DDPM) \cite{ho2022video}. Instead of training on 2D MR data, we perform direct training on 3D data and propose an optimization method that uses under-sampled k-space data to reconstruct 3D MR images. The article is organized as follows: in Section \ref{sec:background} we provide a brief summary of diffusion models as \ac{SDE}, where the connection to \ac{DDPM} as a special case is discussed. Additionally, we also introduce the concept of MR image reconstruction. In Section \ref{sec:methods}, the proposed algorithm for 3D MR image reconstruction is presented. Section \ref{sec:numerics} discusses the numerical experiments including data, model, as well as the comparison of the proposed algorithm with existing methods. To sum up, the discussion and conclusion of our work is presented in Section \ref{sec:conclusion}.  
% % In the following, we discuss the contribution of our work as well as provide the notation used through this article. Figure \ref{Fig:workflow} shows the visualization of the proposed algorithm.
% % \subsection{Summary of Contributions}
% Our contributions can be summarized as follows:
% \begin{itemize}
% \item In order to generate a consistent reconstruction, we propose an optimization algorithm based on the 2D projection of the 3D data to add an additional constraint for the 3D reconstruction. This method is incorporated in the sampling procedure to generate a unique 3D MR image. The key idea stems from the Fourier slice theorem \cite{bracewell1990numerical}, in which showing the relation between axis projection and DC components in the under-sampled k-space. Hence, after training the 3D U-Net, we generate 3D MR images and apply data fidelity from under-sampled k-space with the proposed optimization method.  
% \item In order to optimize 3D image reconstruction, we use a video diffusion model  \cite{ho2022video}. This approach is used to learn the parameter for generative MR images. Since the order of MR images is necessary to produce consistent reconstruction results, we use the order information to train video diffusion model based on a 3D U-Net  for MR image denoising. 
% \item We train this model using the fastMRI knee dataset \cite{zbontar2018fastmri} and MR images of plant roots for plant phenotyping, provided at IBG-2 Jülich Research Center. 
% \item We perform numerical experiments to compare the performance of the proposed algorithmagainst state-of-the art algorithms.We measure the quality of image reconstruction based on several well-known metric evaluations, such as \ac{SSIM} and \ac{PSNR} for both knee  and roots data. All code used in this paper is available: \textcolor{blue}{the link here}
% \end{itemize}
% \begin{figure*}[t!]
%     \centering
%     % \includegraphics[scale=0.8]{Figure/compare_knee.svg}
%     \includegraphics[width=0.95\textwidth]{Figure/3DEyeCatching.pdf}
%     \caption{Workflow of the proposed algorithm generating volumetric data from random distribution and guiding the reconstruction for specific k-space data to have a unique reconstruction}
% \label{Fig:workflow}
% \end{figure*}
% % \subsection{Notations}
% % Vectors  $\mathbf{x} \in \C^L$ and matrices are written in bold small-cap and bold big-cap letter $\mathbf{A} \in \C^{K \times L}$, respectively. A matrix can also be written by indexing its elements, $\mathbf{A} = \left(a_{k\ell}\right), \quad \text{where} \quad k \in [K], \ell \in [L].$ Volumetric data is written as bold italic letter $\textbf{\emph{A}} \in \C^{S \times K \times L}$ or indexing matrix $\mbf{A}_s \,\text{for} \, s \in [S]$. Here we the $\C$ and $\R$ are complex and real field. 
% % The set of integers is written as $[N] := \{1,2,\hdots,N\}$ and calligraphic letters are used to define functions $\mcl{A} : \C \rightarrow \C$. Specifically, we denote the two-dimensional and one-dimensional Fourier transform by $\mathcal{F}_{2D}$ and $\mathcal{F}_{1D}$, respectively.
% % For both matrices and vectors, the notation $\circ$ is used to represent element-wise or Hadamard product. The $\mbf{A}^H$ is used to represent conjugate transpose. For a vector $\mbf x \in \C^L$, the $\ell_p$-norm is given by $\norm{\mbf x}_p = \left(\sum_{\ell = 1}^L \card{x_\ell}^p\right)^{1/p},$ $1 \le p < \infty$ and for $p = \infty$ we have $\underset{\ell \in [L]}{\text{max}} \card{x_\ell}$. %Although it is not a norm, the notation $\norm{\mbf x}_0$ is used to count non-zero elements in a vector. 
% % For a matrix $\mathbf{X} \in \C^{K \times L}$, the Frobenius norm is denoted by $\norm{\mbf X}_F \defeq \sqrt{\sum_{k = 1}^K \sum_{\ell = 1}^L \card{x_{k\ell}}^2} $. 
% % %The time index for \ac{SDE} for vector is written in subscript, i.e, $\mbf{x}_t$ and for each slice matrix from volume data, the subscript index represent index slice and superscript index is the time \ac{SDE}, i.e.,$\mbf{X}^t_s$ for $s \in [S]$. Additionally, the superscript index bracket represents the iterative index, i.e., $\mbf{X}^{(i)}$.




==> Section/method_old.tex <==
\section{Methods and Algorithms}\label{sec:methods}
We first briefly review the diffusion model in section \ref{sec:diffusion_model} and \ac{MRI} reconstruction in section \ref{sec:mri_recon}. In \ref{sec:proposed_method} we present the proposed method.
The notations used throughout this article are summarized below.

% \subsection{Notations} \label{sec:notations}
\paragraph{Notations} \label{sec:notations}
Vectors  $\mathbf{x} \in \C^L$ and matrices are written in bold small-cap and bold big-cap letter $\mathbf{A} \in \C^{K \times L}$, respectively. %A matrix can also be written by indexing its elements, $\mathbf{A} = \left(a_{k\ell}\right), \quad \text{where} \quad k \in [K], \ell \in [L].$ 
Volumetric data is written as bold italic letter $\textbf{\emph{A}} \in \C^{S \times K \times L}$ or indexing matrix $\mbf{A}_s \in \C^{K \times L} \,\text{for} \, s \in [S]$. Here the $\C$ and $\R$ are complex and real fields. 
The set of integers is written as $[N] := \{1,2,\hdots,N\}$. We denote the two-dimensional and one-dimensional Fourier transform by $\mathcal{F}_{2D}$ and $\mathcal{F}_{1D}$, respectively.
For both matrices and vectors, the notation $\circ$ is used to represent element-wise or Hadamard product. %The $\mbf{A}^H$ is used to represent conjugate transpose. For a vector $\mbf x \in \C^L$, the $\ell_p$-norm is given by $\norm{\mbf x}_p = \left(\sum_{\ell = 1}^L \card{x_\ell}^p\right)^{1/p},$ $1 \le p < \infty$ and for $p = \infty$ we have $\underset{\ell \in [L]}{\text{max}} \card{x_\ell}$. %Although it is not a norm, the notation $\norm{\mbf x}_0$ is used to count non-zero elements in a vector. 
For a matrix $\mathbf{X} \in \C^{K \times L}$, the Frobenius norm is denoted by $\norm{\mbf X}_F \defeq \sqrt{\sum_{k = 1}^K \sum_{\ell = 1}^L \card{x_{k\ell}}^2} $. %Finally, the gradient of $\mbf x$ is written as $\nabla_{\mbf x}$.
%The time index for \ac{SDE} for vector is written in subscript, i.e, $\mbf{x}_t$ and for each slice matrix from volume data, the subscript index represent index slice and superscript index is the time \ac{SDE}, i.e.,$\mbf{X}^t_s$ for $s \in [S]$. Additionally, the superscript index bracket represents the iterative index, i.e., $\mbf{X}^{(i)}$.
\subsection{Diffusion Model} \label{sec:diffusion_model}
%\textcolor{red}{
%\begin{itemize}
%    \item Reduce this section, no need too detail    
%\end{itemize}
%}
 We follow the notation in terms of a one-dimensional vector as suggested in the literature \cite{song2020score}.
%A prevalent generative modeling technique is constructing the model as a diffusion process in terms of \ac{SDE} \cite{song2020score}. 
The key idea in the generative model is to learn training data distribution, i.e., image, such that we can generate new images corresponding to the learned distribution.
\paragraph{Training.} In \ac{DDPM} \cite{ho2020denoising, ho2022video}, estimating data distribution can be performed by perturbing the training data with a sequence of positive noise scale $0 < \beta_1, \beta_2, \hdots, \beta_T < 1$ as  follows 
$$
\mbf{x}_t = \sqrt{1 - \beta_t} \mbf{x}_{t-1} + \sqrt{\beta_t} \mbf{z}_{t-1},\,\text{for}\, t \in \{1,2, \hdots, T \}
$$
where $\mbf{z} \sim \mcl{N}\left(\bs{0}, \mbf{I} \right)$.  %this can be achieved by  data distribution to estimate this entity by approximating it with Gaussian conditional probability $p_{t}\left( \mbf{x}_t| \mbf{x}_{t-1} \right)$. 
In this case, the original data $\mbf{x}_0 \sim p_{\text{data}}\left(\mbf x\right)$ is perturbed by a random Gaussian vector with increased variance for each time index. Hence, for each time step of perturbation, the neural network model $\mcll{s}_{\bs \theta}$, for instance, the U-Net architecture, is trained to approximate the conditional distribution from perturbed data.

\paragraph{Sampling.} The pre-trained neural network model $\mcll{s}_{\bs \theta^*} $ is used later to remove the perturbation aspect in order to generate an image similar to the training data distribution. The sampling\footnote{In this article the term sampling should not be confused with undersampling in MRI definition. Here sampling in the generative model describes generating data from a certain probability distribution.} procedure is usually performed, for instance with the Euler-Maruyama scheme, as procedure, as follows:
\begin{multline}
\mbf{x}_{t-1} = \frac{1}{\sqrt{1 - \beta_t}} \left(\mbf{x}_t + \beta_t \mcll{s}_{\bs \theta^*} \left(\mbf{x}_t,t\right) \right) + \sqrt{\beta_t} \mbf{z}_t \\ \,\text{for}\, t \in \{T,T-1,\hdots,1 \},
\label{eq:sampling}
\end{multline}
It should be noted that, the index is reversed because we perform reverse process in the sampling mechanism. For the complete derivation, we refer the interested reader to the literature and references therein \cite{song2020score,ho2020denoising, ho2022video}.

\subsection{3D \ac{MRI} Reconstruction} \label{sec:mri_recon}
We first present the conventional 2D reconstruction for full sample k-space data and develop the model for under-sampled measurement. Afterward, we will discuss the challenge of 3D MRI reconstruction.
\paragraph{Full and Under-sampled Reconstruction.}
The relation between fully sampled k-space and the image space, i.e., image of interest,  in \ac{MRI} is given by the %two-dimensional 
Fourier transform \cite{slichter2013principles, lin2021artificial, knoll2020deep}. Suppose we acquire $S$ single-coil slices of a fully sampled k-space image $\mbf Y_s \in \C^{N_y \times N_x}$ for $s \in [S]$.   Hence, the direct reconstruction in image space can be written as
\begin{equation}
    \mbf{X}_s = \mcl{F}^{-1}_{2D}\left( \mbf{Y}_s \right) \quad \text{for} \quad s \in [S].
\end{equation}

Accelerating \ac{MRI} acquisition is achieved by reducing the number of scan lines during k-space acquisition. As a result, under-sampled k-space is recorded with fewer data points.  We can write this as
\begin{equation}
    \label{eq:forward_model}
    \hat{\mbf{X}}_s =\mcl{F}^{-1}_{2D}\left(  \mbf{M} \circ {\mbf{Y}}_s  \right) \quad \text{for} \quad s \in [S],
\end{equation}
where the matrix $\hat{\mbf{Y}}_s =  \mbf{M} \circ {\mbf{Y}}_s $ and $\hat{\mbf{X}}_s $ are the noisy under-sampled k-space and the reconstruction, called zero-filled image for all slices, respectively. Applying a two-dimensional inverse Fourier transform directly on under-sampled k-space yields low-quality reconstructed images %poses a challenge 
as it results in aliasing and ambiguities.

\paragraph{Challenges in 3D reconstruction.} \label{sec:Challenge3D}
It should be straightforward to construct the 3D image by stacking slice-by-slice reconstruction. However, as discussed in \cite{chung2023solving}, the under-sampled k-space could yield inconsistencies in reconstruction for the $z-$ axis direction. Additionally, reconstruction for the data that have sparse structures in all directions, such as roots and angiography, stacking slice-by-slice reconstruction can also yield non-smoothness in all possible directions. One way to address this problem is by adding constraints in the reconstruction algorithm such that the continuity on $z-y$, $x-z$, as well as $x-y$ can be pertained. Here, we will use the knowledge of projection of 3D data on the image space and its relation to the k-space by using the Fourier slice theorem, as described in Appendix \ref{sec:FourierSlice}. The visualization can be seen in Figure \ref{Fig:projection_image}

\subsection{Proposed Method} \label{sec:proposed_method}
 In this article, we propose an optimization method by incorporating the Fourier slice theorem \cite{bracewell1990numerical, bracewell1956strip} to provide information about the 2D-projected image and its relation to the zero frequency of measurement data (k-space). The algorithm allows us to reconstruct 3D MRI data with enhanced continuity on the $z-$axis using a pre-trained Diffusion Model, i.e. the algorithm is only applied during the sampling process.
 \paragraph{Fourier slice theorem.}
 Suppose we have 3D k-space data given as $\mbf{Y}_s \in \C^{N_y \times N_x}$ for all depth slices $s \in [S]$. The zero frequency of k-space at $x-$axis\footnote{Since the matrix represents the image per slice, the zero frequency on $x-$ and $y-$ axis is given in the middle of row or column space}, i.e., $k_x = 0$, can be written as $  {\mbf{y}}_s^{k_y} = \mbf{Y}_s \vert_{\left(k_x = 0\right)} \in \C^{N_y}$, here we use superscript $k_y$ to inform that this vector is obtained for $k_x = 0$. Additionally, the projection of the 3D image space on the $y-$ axis is given by summing in $x-$direction, i.e.
%
${x}_{s,i} = \mcl{P}_{y}\left(\mbf{X}_s\right)|_i =  \sum_{j = 1}^{N_x} x_{s,i,j} \in \C$.  From the Fourier slice theorem, we can write as follows
$$
{\mbf{y}}_s^{k_y} = \mcl{F}_{1D}\left( \mbf{x}_s\right) \in \C^{N_y},
$$
where $\mcl{F}_{1D}$ is the one-dimensional Fourier transform. Therefore, if we collect the projected vector from all depth slices, i.e., $z$-axis, we construct a matrix with dimension $S \times N_y$. The same concept can be adopted to get the projected image space on $x$-axis from projecting function $\mcl{P}_{x}$. It should be noted that in many cases we have the same dimension for each slice, i.e., $N_y = N_x = N$, hence, the dimension of volumetric data is in the form of $S \times N \times N$. Additionally, in order to incorporate the undersampling operator we can write $ \mbf{m}^{k_y}= \mbf{M} \vert_{\left(k_x = 0\right)} \in \C^{N_y}$ is the slice of the under-sampling operator at $k_x = 0$. Hence, we have
\begin{equation}
     \hat{\mbf{y}}_s^{k_y} = \mbf{m}^{k_y} \circ \mcl{F}_{1D}\left( \mbf{x}_s\right) \in \C^{N_y} \quad  \text{for}\quad s \in [S].
\end{equation}
\Cref{Fig:projection_image} visualizes the concept of projected volume data to image space and its relation to Fourier transform.
\begin{figure}[tb]
\centering
    \includegraphics[width=0.45\textwidth]{Figure/update_proj_mri.pdf}
    % \includesvg[width=0.45\textwidth]{Figure/update_proj_mri.svg}
    \caption{Relation between the projected image and a slice of k-space from plant roots data}
\label{Fig:projection_image}
\end{figure}
\paragraph{Optimization problem.}
From this information, we can form an optimization problem to reconstruct three-dimensional images from under-sampled k-space, as follows:
\begin{equation}
\small
\underbrace{\begin{aligned}
\label{eq:opt}
 \textbf{\emph X$^*$} = &\underset{\textbf{\emph X} \in \C^{S \times N \times N}}{\text{arg min}}
& & 
\sum_{s = 1}^S \norm{\hat{\mbf{Y}}_s - \mbf{M} \circ \left( \mcl{F}_{2D}\left( \mbf{X}_s \right)\right) }_F^2
\tikzmarkend{a-1}
+ \mcl{R}\left(\textbf{\emph X} \right) \\
& \text{subject to}
& & \hat{\mbf{y}}_s^{k_y} = \mbf{m}^{k_y} \circ \mcl{F}_{1D}\left( \mcl{P}_{y} \left(\mbf{X}_s\right)\right) \quad  \text{for } s \in [S]\\
&&& \hat{\mbf{y}}_s^{k_x} =  \mbf{m}^{k_x} \circ \mcl{F}_{1D}\left( \mcl{P}_{x} \left(\mbf{X}_s\right)\right) 
\end{aligned}}_{\mcl{G}\left(\textbf{\emph X} \right)}
\end{equation}
The regularization functions $\mcl{R}\left(\textbf{\emph X}\right)$ used in this article can be written as
\begin{equation}
\label{eq:reg}
\begin{aligned}
  &\alpha \underbrace{\sum_{s=1}^S\sum_{i=1}^N\sum_{j=1}^N \card{x_{s,i,j}}}_{\text{sparsity}} +\underbrace{\sum_{s=1}^S \sum_{i=1}^N\sum_{j=1}^{N-1}  \card{x_{s,i,j+1} - x_{s,i,j}}^2}_{\text{smoothness}}  \\&+  \underbrace{\sum_{s=1}^S\sum_{i=1}^{N-1}\sum_{j=1}^{N} \card{x_{s,i + 1,j} - x_{s,i,j}}^2}_{\text{smoothness}} 
\end{aligned}
\end{equation}
In general, the optimization problem $\mcl{G}\left(\textbf{\emph X} \right)$ as in \eqref{eq:opt} describes the objective and constraint functions to estimate three-dimensional image space given the relation between its under-sampled three-dimensional k-space and the projection from the Fourier slice theorem. This ensures the reconstructed image corresponds to the given measurement. In addition, we have regularization for each element of volumetric data in terms of $\ell_1$-norm, left side constraint in \eqref{eq:reg}. and the approximated total variation norm, right side constraint in \eqref{eq:reg}. These terms are used for imposing the result with certain structures, i.e., sparsity or smoothness \cite{parikh2014proximal, rudin1992nonlinear}. The importance of the regularization terms is discussed in Section \ref{Sec:Ablation}.
In general, the optimization problem $\mcl{G}\left(\textbf{\emph X} \right)$ as in \eqref{eq:opt} describes the objective and constraint functions to estimate three-dimensional image space given the relation between its under-sampled three-dimensional k-space and the projection from the Fourier slice theorem. This ensures the reconstructed image corresponds to the given measurement. In addition, we have regularization for each element of volumetric data in terms of $\ell_1$-norm, left side constraint in \eqref{eq:reg}. and the approximated total variation norm, right side constraint in \eqref{eq:reg}. These terms are used for imposing the result with certain structures, i.e., sparsity or smoothness \cite{parikh2014proximal, rudin1992nonlinear}. The importance of the regularization terms is discussed in Section \ref{Sec:Ablation}.
In general, the optimization problem $\mcl{G}\left(\textbf{\emph X} \right)$ as in \eqref{eq:opt} describes the objective and constraint functions to estimate three-dimensional image space given the relation between its under-sampled three-dimensional k-space and the projection from the Fourier slice theorem. This ensures the reconstructed image corresponds to the given measurement. In addition, we have regularization for each element of volumetric data in terms of $\ell_1$-norm, left side constraint in \eqref{eq:reg}. and the approximated total variation norm, right side constraint in \eqref{eq:reg}. These terms are used for imposing the result with certain structures, i.e., sparsity or smoothness \cite{parikh2014proximal, rudin1992nonlinear}. The importance of the regularization terms is discussed in Section \ref{Sec:Ablation}.

In practice, the implementation can be performed in terms of alternating minimization combined with some proximal methods for the regularization function. Note that the $\ell_1$-norm constraint is non-smooth, the proximal method is used to avoid calculating its derivative. The analytic proximal of $\ell_1$-norm is well known, namely soft thresholding function  \cite{bolte2014proximal, parikh2014proximal, foucart2013mathematical}, which is also presented in Appendix \ref{Sect:Prox_Regul}. Hence, the algorithm can be seen as applying proximal on the gradient update of the loss function by putting all constraints in the optimization \eqref{eq:opt} as a single loss equation, which is also called proximal gradient method \cite{bolte2014proximal, parikh2014proximal}, the implementation detail will be presented in Appendix \ref{Sect:Prox_Regul}. 
\paragraph{Diffusion Fourier Slice Optimization.}
The above optimization steps are inserted in the sampling process of a pre-trained Diffusion Model. Therefore, the proposed algorithm, namely the Diffusion Fourier Slice Optimization, consists of two parts. The Diffusion Model part provides the data-related prior knowledge. The Fourier Slice Optimization incorporates the k-space measurement to ensure the fidelity of the generated data. In addition, the regularisation term in \eqref{eq:reg} gives general prior knowledge of the MRI data, i.e. sparsity and smoothness. 
% can be implemented by combining the inference or sampling process of \ac{DDPM} and the Fourier Slice Optimization in \eqref{eq:opt}, which yields a combination between image generation and data fidelity from the optimization method given under-sampled k-space data. 

The overall algorithm is described in Algorithm \ref{algo:DDPM_Sampling_Proximal}. The algorithm starts with generating a 3D MRI image via the sampling process of \ac{DDPM}, which is guided by the Fourier Slice Optimization in \eqref{eq:opt} to incorporate the under-sample k-space, i.e., to reconstruct a specific 3D MRI image from the k-space measurement. It should be noted that the superscript $(i)$ and subscript index $t$ is used to denote the iteration index between both optimization update and the \ac{DDPM} sampling. Hence, the algorithm performs \ac{DDPM} sampling and optimization updates alternatingly.
\begin{algorithm}
% \scriptsize
    \caption{\ac{DDPM} Sampling with Fourier Slice Optimization}
    \label{algo:DDPM_Sampling_Proximal}
    \begin{algorithmic}[1]
        \State \textbf{Initialization:} 
        \begin{itemize}
            \item Timesteps $T$ and optimization iterations $m$
            \item Volume sampling from prior distribution $ {\textbf{\emph X}_{T}} \in \R^{S \times N \times N} \sim \mcl{N}\left(\bs{0},\mbf{I}\right)$ 
        \end{itemize}
        \For{each reverse iteration $t = T \quad \textbf{to} \quad 1 $ }
            \State Generate $\textbf{\emph Z}  \sim \mcl{N}\left(\bs{0},\mbf{I}\right)$ if $t > 1$ else $\textbf{\emph Z} = \bs{0}$  
            \State Update sample {(\ref{eq:sampling})} $$
            \textbf{\emph X}^{\left(0\right)} = \frac{1}{\sqrt{1 - \beta_t}} \left(\textbf{\emph X}_t + \beta_t \mcll{s}_{\bs \theta^*} \left(\textbf{\emph X}_t,t\right) \right) + \sqrt{\beta_t} \textbf{\emph Z}_t 
            $$
            {\For{each iteration $i = 1 \quad \textbf{to} \quad m $ } 
                \State{\parbox[t]{\dimexpr\linewidth-\algorithmicindent}{%
          Solving the optimization\\ problem in \eqref{eq:opt}\\
          $\textbf{\emph X}^{\left(i\right)} = \mcl{G}\left(\textbf{\emph X}^{\left(i-1\right)}\right)$
        }}
                
                %$$
                %\textbf{\emph X}^{\left(i\right)} =  \text{prox}_{\alpha} \left(\textbf{\emph X}^{\left(i-1\right)} - \lambda \nabla_{\textbf{ \emph X}^{\left(i-1\right)}} \widehat{L}\left(\textbf{\emph X}^{\left(i-1\right)},  \rho \right)  \right),
                %$$
                %\State where the loss function $\widehat{L}\left(\textbf{\emph X},  \rho \right) $ is given in \eqref{eq:loss_function}
            \EndFor
            \State $\textbf{\emph X}_{t-1} = \textbf{\emph X}^{\left(m\right)} $}
        \EndFor\\
        \Return ${\textbf{\emph X}}_0 \in \C^{S \times N \times N}$
        %\EndProcedure
    \end{algorithmic}
\end{algorithm}
%by transforming continuously from one data distribution $\mbf{x}_0 \sim p_{0}\left(\mbf x \right)$ to another distribution $\mbf{x}_T \sim p_T\left(\mbf x \right)$ that is tractable to sample from, i.e., Gaussian distribution. In the literature, this process is also called {forward}  \ac{SDE}. The process can be done progressively and modeled as the solution to the \ac{SDE} with respect to time index $t \in [0, T]$, as follows: 
%\begin{equation}
%\label{eq:forward_SDE}
%    \mrm{d}\mbf{x} = \mcll{f}\left(t, \mbf{x} \right)  \mrm{d}t + \mcll g \left( t \right) \mrm{d}\mbf{w},
%\end{equation}
%where according to the definition of \ac{SDE} the variable $\mbf{w}$ is the standard Wiener process, i.e., Brownian motion and the functions $\mcll{f}: \R^N \rightarrow \R^N$ and $\mbf \mcll{g}: \R  \rightarrow\R$ are drift and diffusion coefficients of $\mbf{x}_t$, respectively.

%The reverse of a diffusion process can be generated by starting from the sample of distribution $\mbf{x}_T\sim p_T\left(\mbf x \right)$ in order to construct the sample according to data distribution $\mbf{x}_0 \sim p_0\left(\mbf x \right)$. The reverse-time process can be described as\cite{anderson1982reverse, song2020score}:
%\begin{equation}
%\label{eq:reverse_SDE}
%    \mrm{d}\mbf{x} = \left( \mcll{f}\left(\mbf{x}, t \right) \mrm{d}t - \mcll{g}^2\left( t \right)  \nabla_{\mbf x} \log p_t\left(\mbf{x} \right) \right)+ \mcll{g}\left( t \right) \mrm{d}\mbf{w}.
%\end{equation}
%In the {reverse} \ac{SDE} process, we apply the drift and diffusion coefficients from the forward \ac{SDE} in \eqref{eq:forward_SDE} with addition of score function $\nabla_{\mbf x} \log p_t\left(\mbf{x} \right)$ for each time index $t \in [0, T]$. 
%The score function $\nabla_{\mbf x} \log p_t\left(\mbf{x} \right)$ is unknown and can be seen as the gradient of the data distribution with respect to the time index. Denoising Score Matching \cite{vincent2011connection, song2020score} and Denoising Diffusion Probabilistic Models \cite{ho2020denoising, ho2022video} try to estimate this entity by approximating it with Gaussian conditional probability $p_{t}\left( \mbf{x}_t| \mbf{x}_{t-1} \right)$. In this case, the original data $\mbf{x}_0 \sim p_{\text{data}}\left(\mbf x\right)$ is perturbed by a random Gaussian vector with increased variance for each time index. We briefly discuss the \ac{DDPM} approach since we will leverage it in this article. Suppose we have training data $\mbf{x}_0 \sim p_{\text{data}}\left(\mbf x \right)$ and perturb the data with a sequence of positive noise scale $0 < \beta_1, \beta_2, \hdots, \beta_T < 1$ as  follows 
$$
%\mbf{x}_t = \sqrt{1 - \beta_t} \mbf{x}_{t-1} + \sqrt{\beta_t} \mbf{z}_{t-1},\,\text{for}\, t \in \{1,2, \hdots, T \}
$$
%where $\mbf{z} \sim \mcl{N}\left(\bs{0}, \mbf{I} \right)$. This perturbation strategy is a discrete version of forward \ac{SDE}, where for \ac{DDPM} the drift and diffusion coefficients for continuous time are given by parameter $\beta$, as discussed in \cite[eq.22-25]{song2020score}:
%$$
% \mrm{d}\mbf{x} = -\frac{1}{2}\beta(t) \mbf{x} \mrm{d}t + \sqrt{\beta(t)}  \mrm{d}\mbf{w},
%$$
%Hence, for each time step, we have a conditional probability $p\left(\mbf{x}_t | \mbf{x}_{t-1}\right) = \mcl{N}\left(\mbf{x}_t; \sqrt{1-\beta_t}\mbf{x}_{t-1},\beta_t \mbf{I} \right)$ or the conditional probability that contains the original data $\mbf{x}_0$, i.e., $p_{\alpha_t}\left(\mbf{x}_t | \mbf{x}_{0}\right) = \mcl{N}\left(\mbf{x}_t; \sqrt{\alpha_t}\mbf{x}_{0},(1 -  \alpha_t) \mbf{I} \right)$, where $\alpha_t = \prod_{j=1}^t (1- \beta_j)$. The distribution of perturbed data for each time index can be calculated as $p_{\alpha_t}\left(\tilde{\mbf{x}}  \right) = \int p_{\text{data}}\left(\mbf x \right) p_{\alpha_t}\left(\tilde{\mbf{x}} | \mbf{x} \right)  \mrm{d} \mbf{x}$. The neural network model $\mcll{s}_{\bs \theta}$  is trained to approximate  the gradient of conditional distribution from perturbed data for each time step with the following loss:
%\begin{equation}
%    \bs \theta^* = \underset{\bs \theta}{\text{arg min}}  \sum_{t = 1}^T (1 - \alpha_t) \E_{p_{\text{data}}\left(\mbf x\right)}\E_{p_{\alpha_t}\left(\tilde{\mbf{x}}|\mbf{x}\right)}\left[ \norm{\mcll{s}_{\bs \theta} \left(\tilde{\mbf{x}},t\right)  - \nabla_{\tilde{\mbf x}} \log  p_{\alpha_t}\left( \tilde{\mbf{x}}| \mbf{x}\right)}_2^2 \right]
%    \label{eq:loss}
%\end{equation}

%fter finding optimal parameters $\theta^*$ the reverse \ac{SDE} incorporating with noise $\mbf{z} \sim \mcl{N}\left(\bs{0}, \mbf{I} \right)$ is performed by sampling\footnote{In this article the term sampling should not be confused with undersampling in MRI definition. Here sampling in the generative model describes generating data from a certain probability distribution.} procedure, as follows:
%\begin{equation}
%\mbf{x}_{t-1} = \frac{1}{\sqrt{1 - \beta_t}} \left(\mbf{x}_t + \beta_t \mcll{s}_{\bs \theta^*} \left(\mbf{x}_t,t\right) \right) + \sqrt{\beta_t} \mbf{z}_t ,\,\text{for}\, t \in \{T,T-1,\hdots,1 \},
%\label{eq:sampling}
%\end{equation}
%which is a discrete version of reverse \ac{SDE} with DDPM approach.
% HS: moved this definition up
%, where $\mbf{z} \sim \mcl{N}\left(\bs{0}, \mbf{I} \right)$. 
%The complete derivation is given in \cite[Appendix E]{song2020score}.  
%The summary of \ac{DDPM} sampling algorithm is presented in  Algorithm \ref{algo:DDPM Sampling}.
%\begin{algorithm}
%\caption{\ac{DDPM} Sampling \cite{ho2020denoising,song2020score}}
%\label{algo:DDPM Sampling}
%\begin{algorithmic}[1]
%\State \textbf{Initialization:} 
%\begin{itemize}
%    \item Number of time step $T$
%    \item Sampling from prior distribution ${\mbf{\hat   x_{T}}} \sim \mcl{N}\left(\bs{0},\mbf{I}\right)$
%\end{itemize}
%\For{each iteration $t = T, T-1 \quad \textbf{to} \quad 1 $ }
%\State Generate $\mbf{z} \sim \mcl{N}\left(\bs{0},\mbf{I}\right)$ if $t > 1$ else $\mbf{z} = \bs{0}$  
%\State Update sample
$$
%\mbf{x}_{t-1} = \frac{1}{\sqrt{1 - \beta_t}} \left(\mbf{x}_t + \beta_t \mcll{s}_{\bs \theta^*} \left(\mbf{x}_t,t\right) \right) + \sqrt{\beta_t} \mbf{z}_t
$$
%\EndFor
%\State \Return $\hat{\mbf{x}}_0$
%\EndProcedure
%\end{algorithmic}
%\end{algorithm}

% \vspace{-2cm}
%\begin{itemize}
%    \item Discuss the current problem with 3D reconstruction
%    \item Limitation of stacking slice by slice
%    \item Computation time?
%    \item Write strong motivation why Fourier Slice and the proximal proj method are important
%\end{itemize}
%}
%Furthermore, with under-sampled k-space data, the proposed reconstruction algorithm should also perform comparable image quality to the full-scan reconstruction and yield consistent reconstruction in all directions.  

%Combining the information provided from k-space with reverse sampling in the diffusion model, the image can be uniquely reconstructed by rewriting the score function in \eqref{eq:reverse_SDE} with a posterior distribution.

%From Bayesian perspective, we can write the this problem as Bayesian inference problem, where we would like to estimate the posterior distribution $p\left(\mbf{X}| \hat{\mbf{Y}}\right)$. Hence, if we want to incorporate the  {reverse} \ac{SDE} for \ac{MRI} reconstruction, the score function in \eqref{eq:reverse_SDE} should be replaced by $\nabla_{\mbf X} \log p\left(\mbf{X}| \hat{\mbf{Y}}\right)$ or specifically its expansion by using Bayes rule:
%\begin{equation}
%    \nabla_{\mbf X} \log p\left(\mbf{X}| \hat{\mbf{Y}}\right) = \nabla_{\mbf X} \log p\left(\hat{\mbf{Y}}|\mbf{X}\right) + \nabla_{\mbf X} \log p\left(\mbf{X}\right).
%\end{equation}
%There are at least two benefits of this reformulation. Firstly, we can apply a pre-trained score model to approximate the score function $\nabla_{\mbf X} \log p\left(\mbf{X}\right)$. Secondly, the function $\nabla_{\mbf X} \log p\left(\hat{\mbf{Y}}|\mbf{X}\right)$ can be seen as gradient of log-likelihood from Gaussian distribution and acts as gradient step in the optimization scheme. In Section \ref{sec:proposed_method}, we will discuss the proposed algorithm to approximate $\nabla_{\mbf X} \log p\left(\hat{\mbf{Y}}|\mbf{X}\right)$ combining with the sampling procedure for {reverse} \ac{SDE} that approximates $\nabla_{\mbf X} \log p\left( \mbf{X}\right)$.

%
% For a matrix $\mbf{X} \in \C^{N_y \times N_x}$, the projection is defined as follows:
%\begin{equation}
%\begin{aligned}
%\mcl{P}_{y}\left(\mbf{X}\right) &= \left( \sum_{j = 1}^{N_x} x_{1,j},  \sum_{j = 1}^{N_x} x_{2,j},\hdots, \sum_{j = 1}^{N_x} x_{N,j} \right)^T \in \C^{N_y}
%\end{aligned}
%\end{equation}
%\textcolor{black}{The proximal method can be seen as the constraint applied to the data that we want to estimate, such that the reconstructed data have a structure according to the solution we want to have, i.e., sparsity and smoothness.}
%It should be noted that depending on the regularization that we impose on the optimization variable $\mbf{X}_s$ we have different functions for proximal method. For instance, in sparsity we have soft thresholding operator as proximal function for $\ell_1-$norm \cite[eq.15.22]{foucart2013mathematical}. 



==> Section/references.tex <==
%\bibliographystyle{IEEEbib}
%\bibliographystyle{unsrt}

\bibliography{IEEEabrv,references}
